Streaming Algorithms for Support-Aware Histograms

Histograms, i.e., piece-wise constant approximations, are a popular tool used to represent data distributions. Traditionally, the difference between the histogram and the underlying distribution (i.e., the approximation error) is measured using the $L_p$ norm, which sums the differences between the two functions over all items in the domain. Although useful in many applications, the drawback of this error measure is that it treats approximation errors of all items in the same way, irrespective of whether the mass of an item is important for the downstream application that uses the approximation. As a result, even relatively simple distributions cannot be approximated by succinct histograms without incurring large error. In this paper, we address this issue by adapting the definition of approximation so that only the errors of the items that belong to the support of the distribution are considered. Under this definition, we develop efficient 1-pass and 2-pass streaming algorithms that compute near-optimal histograms in sub-linear space. We also present lower bounds on the space complexity of this problem. Surprisingly, under this notion of error, there is an exponential gap in the space complexity of 1-pass and 2-pass streaming algorithms. Finally, we demonstrate the utility of our algorithms on a collection of real and synthetic data sets.

==> background.tex <==
\section{Learning Histograms}

\paragraph{Setup}
\begin{itemize}
    \item Goal: estimate density of a distribution (e.g., corresponding to the empirical frequency distribution in a stream) using $k$-piece histogram
    \item Sampling + Eval query access to the distribution
    \item Error measured as $\ell_1$ error on the support of target distribution (rather than over the whole domain)
\end{itemize}

\subsection{Background}

\paragraph{$L_p$ Sampling}
From Jayaram-Woodruff \url{https://arxiv.org/pdf/1808.05497.pdf} (see also survey by Cormode-Jowhari \url{https://wp.kntu.ac.ir/jowhari/papers/Lpsurvey.pdf}), we can get perfect $L_p$ sampling + approximate Eval queries in time 
\[
    O(\log^2 n \log \delta^{-1} + \eps^{-p} \log n)
\]
for $p \in (0,2)$.

\paragraph{Tolerant testing with Eval queries (over domain)}
From Canonne-Rubinfeld \url{https://arxiv.org/pdf/1402.3835.pdf}, suppose we have some known distribution $Q$ and sample/eval access to a distribution $P$ (both discrete distributions over $[n]$).
We can express the total variation distance between $P$ and $Q$ as follows:
\begin{align*}
    d_{TV}(P, Q) &= \frac{1}{2} \sum_{i=1}^n \left| P(i) - Q(i) \right|
    = \sum_{i: P(i) > Q(i)} \left(P(i) - Q(i)\right) \\
    &= \sum_{i: P(i) > Q(i)} \left(1 - \frac{Q(i)}{P(i)}\right) P(i) \\
    &= \E_{i \sim P} \left[\left(1 - \frac{Q(i)}{P(i)}\right) \1 [P(i) > Q(i)] \right].
\end{align*}
As the elements of the expectation are in $[0,1]$, if we randomly sample $i \sim P$, by Chernoff bounds we can estimate the distance between $P$ and $Q$ up to $\eps$ using $O(\eps^{-2})$ samples with constant success probability.

If we parameterize histograms by choosing $k-1$ breakpoints and choosing values for each piece from a grid with resolution $O(\frac{\eps}{k})$, then there are $O(\binom{n}{k} (k/\eps)^k)$ possible histograms.
So, with an additional $O(k \log nk\eps^{-1})$ factor, we can estimate the distance between all histograms (defining $Q$) and $P$ up to $\eps$ with constant failure probability by union bound and thus will find an approximately optimal histogram, up to additive error $2\eps$ (with exponential runtime).

As noted in the Canonne-Rubinfeld paper, if we have a multiplicative approximate Eval queries (as we get with $L_p$ sampling), everything goes through with some minor adjustments to the error parameter.

\paragraph{Learning Histograms over Domains (with no Eval queries)}
From CDSS \url{https://arxiv.org/pdf/1411.0169.pdf}, using $\tilde{O}(k/\eps^2)$ samples and time, they can get a $O(k\log^2(1/\eps))$-piece histogram that has total variation distance at most
\[
    C*\text{opt}_k + \eps
\]
from the true density whp, where $\text{opt}_k$ is the error of the best $k$-piece histogram.

While the algorithm based on the tolerant tester with Eval queries takes exponential time, it has the same sample complexity up to logarithmic factors, uses exactly $k$ pieces, and has \emph{no multiplicative error}. Note that without Eval queries, CDSS show that $C > 1.99$ for any algorithm using $o(\sqrt{N})$ samples: the multiplicative error is necessary.

\subsection{Error over support}

\paragraph{What changes when we focus on error over support?}
\begin{itemize}
    \item Restricting our histogram to be a distribution over the same domain as the distribution we are trying to estimate (which both CR and CDSS do) no longer makes sense. Consider the distribution that is uniform over a constant number $c$ of points in domain $[n]$. The $1$-piece histogram that assigns weight $1/c$ to all points is optimal even though its total mass over the domain is $n/c >> 1$.
\end{itemize}
Formally, before we had a distribution $P$ that we want to estimate by some piecewise-constant distribution $Q$ with the following error metric:
\begin{equation}
    d_{TV}(P, H) = \frac{1}{2} \sum_{i=1}^n |P(i) - Q(i)|.
\end{equation}
Now in the support case, we want to estimate $P$ by some piecewise-constant function $h$ with error:
\begin{equation}
    d_{supp}(P,h) = \sum_{i: P(i) > 0} |P(i) - h(i)|.
\end{equation}

\paragraph{Tolerant testing with Eval queries (over support)}
Can we adapt the CR tester for the support case?
The key in the CR tester was to express the distance between $P$ and $H$ as an expectation over $i \sim P$ with terms in the expectation being in $[0,1]$ so we could estimate the distance by sampling from $P$ and apply Chernoff bounds.
We can express $d_{supp}(P,h)$ as an expectation in terms of $i \sim P$, but the terms are no longer bounded:
\begin{align*}
    d_{supp}(P, h) &= \sum_{i: P(i) > 0} |P(i) - h(i)| = \sum_{i: P(i) > 0} \left|1 - \frac{h(i)}{P(i)} \right| P(i)\\
    &= \E_{i \sim P} \left|1 - \frac{h(i)}{P(i)}\right|.
\end{align*}
\emph{This doesn't work.} Consider a distribution $P$ where all but one of the elements in $P$'s support have constant density $c$ with the last element having density $1/n$.
The 1-piece histogram $h(i) = c$ for all $i$ has error $c - 1/n \approx c$.
However, if we see $o(n)$ samples, we are unlikely to see the low probability element and will estimate $d_{supp}(P, h) = 0$.
In the context of concentration bounds, the expectation above for this $P$ will mostly have zero terms but will have one huge term $|1 - cn| \approx cn$, so sampling will have high variance.

What if we instead consider the distribution case where we want to estimate $d_{supp}(P,Q)$ for some known distribution (over the domain) $Q$?
Then,
\[
    d_{supp}(P,Q) = \sum_{i: P(i) > 0} |P(i) - Q(i)| \geq \sum_{i: P(i) > Q(i)} (P(i) - Q(i)) 
\]
and
\[
    d_{supp}(P,Q) = \sum_{i: P(i) > 0} |P(i) - Q(i)| \leq 2 d_{TV}(P,Q) = 2 \sum_{i: P(i) > Q(i)} (P(i) - Q(i)).
\]
Combining these bounds, if we let
\[
    \mu = \E_{i \sim P} \left[\left(1 - \frac{Q(i)}{P(i)}\right) \1 [P(i) > Q(i)] \right],
\]
then
\[
    d_{supp} \in [\mu, 2\mu]
\]
So, we can get an approximation to $d_{supp}$ with multiplicative error $2$ and additive error $\eps$ using the same $O(\eps^{-2})$ estimator as in the domain case.


==> onepasslower.tex <==

\section{Space Lower Bound}
\subsection{Proper learning}
\begin{theorem}
Any streaming algorithm for proper learning of $2$-histograms in our model (error counted only on support, stream allows deletions) requires $\Omega(\sqrt n)$ space.
\end{theorem}
\begin{proof}
We reduce from Augmented Indexing. We recall that Indexing is a one-way communication problem where Alice's input is a bitstring $a_1,...,a_t$, Bob's input is $j\in[t]$, Alice sends one message to Bob, and Bob needs to report  $a_j$ with probability better than $1/2$. In the Augmented Indexing variant, Bob also gets $a_1,\ldots,a_{j-1}$ as part of his input. Both variants are known to require $\Omega(t)$ communication. We set $t=\sqrt n$.

\paragraph{The reduction}
Our universe is $1,\ldots,3n$ where for simplicity $n$ is an integer square. The counts of all items $i=2n+1,\ldots,3n$ are always set to $1$. We partition $1,...,2n$ into $2\sqrt{n}$ equal-size consecutive intervals of length $\sqrt{n}$, and denote them as $A_1,B_1,A_2,B_2,\ldots,A_{\sqrt n}, B_{\sqrt n}$. We think of the $A_j$'s as Alice's cells and of the $B_j$'s as Bob's cells.

\paragraph{Alice's reduction:}
Given her input, for every $j=1,\ldots,\sqrt n$, Alice sets all elements in $A_j$ to $a_j$. So, every $A_j$ contains either no supported elements (if $a_j=0$) or $\sqrt n$ mice (if $a_j=1$). She does it by streaming the appropriate updates into the streaming algorithm, and then sends the memory state to Bob.

\paragraph{Bob's reduction:}
Bob streams into the memory state the following updates:
\begin{enumerate}
  \item He sets all elements in every $A_1,...,A_{j-1}$ to zeros (he knows where the nonzeros are by the Augmented part of Augmented Indexing).
  \item In each $B_1,\ldots,B_{j-1}$, he sets $\frac{\sqrt n}{j - 1}$ of the elements to have mass $\sqrt n$ (elephants). 
  \item In $B_j$, he sets $\gamma\sqrt{n}$ of the elements to have mass $\sqrt n$ (elephants), where $\gamma>\epsilon$ is a small constant.
\end{enumerate}

This concludes the stream. Note that the total count of masses is $O(n)$, the algorithm is guaranteed to return an optimal $2$-histogram up to an additive error of $\epsilon n$. 
Now Bob lets the algorithm find an approximately best $2$-histogram. Wlog, the values of the histogram are either $\sqrt n$ or $1$, since these are the only frequencies in the input. 
If at least half of the elements in $A_j$ are given histogram value $1$, Bob reports $1$, and reports $0$ otherwise.

To show the correctness of the communication protocol, first note that the algorithm has to put one piece with value $\sqrt n$ on the prefix (in order to cover the elephants in $B_1,\ldots,B_{j-1}$) and another piece with value $1$ on the suffix (to cover the mice in $2n+1\ldots,3n$), as otherwise the error is at least $\approx n$, which as we will see momentarily is much larger than the optimum in either case.
So the question is where it places the breakpoint between the two pieces.

Consider the case $a_j=0$. In this case, the optimal solution has zero error: we can cover $A_1,B_1,\ldots,A_j,B_j$ with the $\sqrt{n}$-piece, and the rest with the $1$-piece. 
So, the algorithm must move from the $\sqrt n$-piece to the $1$-piece \textbf{after} $B_j$ (and in particular $A_j$ needs to be covered by the $\sqrt n$-piece), since otherwise, it incurs error $\approx \gamma n$ on $B_j$, which is more than $\epsilon n$. 

Consider the case $a_j=1$. In this case, the optimal solution has error $\approx \gamma n$: we can cover $A_1,B_1,\ldots,A_{j-1},B_{j-1}$ with the $\sqrt n$-piece, and the rest with the $1$-piece, so that the only error we incur is $\approx \gamma n$ on $B_j$. 
So, the algorithm must move from the $\sqrt n$-piece to the $1$-piece \textbf{before} at least half of $A_j$ (and in particular, at least half of $A_j$ needs to be covered by the $1$-piece), since otherwise, it incurs error $\approx \tfrac12 n$ on $A_j$, and the gap from the optimal error $\approx \gamma n$ is more than $\approx \gamma n$ if $\gamma<\tfrac14$. 

So, as long as the algorithm succeeds with probability more than $0.5$, the theorem is proven.
\end{proof}

\subsection{Bicriterion}
\begin{theorem}
Let $\eps < \frac{1}{40}$ be an error parameter and let $opt_k(S)$ be the $\ell_1$ approximation error of the best-fit $k$-piece histogram for the frequency distribution of a stream $S$. 
Any streaming algorithm that outputs a histogram with at most $\sqrt{n}/40$ pieces with approximation error $opt_2(S) + \eps$ must use $\Omega(\sqrt{n})$ space.
\end{theorem}
\begin{proof}
The proof is quite similar to the proper learning lower bound and relies on a reduction from Augmented Indexing.

\paragraph{The reduction}
Assume that we are given an algorithm that satisfies the guarantees in the theorem statement. Given an instance of Augmented Indexing over $\sqrt{n}$ bits, we will show how to solve the problem via the streaming algorithm on a stream over domain size $n$.

Assume for simplicity that $n$ is a perfect square.
We will split the domain of the stream into $\sqrt{n}$ contiguous chunks of size $\sqrt{n}$ called $S_1, \ldots, S_{\sqrt{n}}$.
For some constant $b \in [0,1]$ which we will later define, we will split each chunk $S_i$ into $b \sqrt{n}$ equal size subintervals $S_i^1, \ldots, S_i^{b\sqrt{n}}$. The first index of each subinterval will be reserved for Bob and the rest will be reserved for Alice.

\paragraph{Alice's reduction}
Alice will go through her $\sqrt{n}$ bits of her string $x$ and perform the following stream operations:
\begin{itemize}
    \item If $x_i = 0$, do nothing.
    \item If $x_i = 1$, add $a\sqrt{n}$ mice to chunk $S_i$ for some constant $a \in [0,1]$ in the following way. For each subinterval of $S_i$, pick $\frac{a}{b}\sqrt{n}$ indices other than the first index of the subinterval. Add a singleton element to the stream corresponding to each of these indices.
\end{itemize}
The result on the frequency distribution will be that for all of Alice's bits which equal $1$, there will be $a\sqrt{n}$ elements with mass $1/m$ if $m$ is the total mass of the stream.

\paragraph{Bob's reduction}
Bob has a single index $i$ of interest as well as knowledge of $x_1, \ldots, x_{i-1}$. Bob will execute the following stream updates.
\begin{itemize}
    \item For $j = 1,\ldots, i-1$, Bob will use his knowledge of Alice's bits to delete any elements Alice added in the chunks $S_1, \ldots S_{i-1}$.
    \item For each subinterval of $S_i$, Bob will add $\sqrt{n}$ copies of the first index of the subinterval.
\end{itemize}
The result on the frequency distribution will be that there will be zero mass on $S_1, \ldots S_{i-1}$ and there will be $b\sqrt{n}$ elements with mass $\sqrt{n}/m$ in chunk $S_i$.

After running the streaming algorithm, we will get some histogram approximation of the frequency distribution.
In order to use this to solve the indexing problem, we will do the following post-processing step.
Let $c \in [0,1]$ be some constant with $c < b$ and let the first indices of each of the subintervals of $S_i$ be refered to as as Bob's indices.
\begin{itemize}
    \item If at least $c\sqrt{n}$ of Bob's indices are approximated to have mass at least $\frac{1}{2\sqrt{n}}$, then report that $x_i = 1$.
    \item If at least $c\sqrt{n}$ of Bob's indices are approximated to have mass less than $\frac{1}{2\sqrt{n}}$, then report that $x_i = 0$.
\end{itemize}

Note that the total mass of the stream $m = \theta(n)$. \Justin{(maybe make Alice fix $m = n$ exactly)}
We will proceed by cases to show that if the streaming algorithm has the $\eps + opt_2(S)$ error guarantee in the theorem statement, then Bob will correctly recover Alice's $i$th bit.
For now, we will parameterize the number of pieces the streaming algorithm produces as $k\sqrt{n}$ for some constant $k$.

\paragraph{Case 1: $x_i = 0$.}
In this case, $opt_2(S) = 0$ as we can simply have the first piece of the histogram predict mass $\frac{1}{\sqrt{n}}$ for chunks $S_1,\ldots, S_i$ and predict mass $\frac{1}{n}$ for chunks $S_{i+1}, \ldots, S_{\sqrt{n}}$. As Alice and Bob's elements do not overlap, two pieces suffice to perfectly approximate the frequency distribution.

Assume that at least $c\sqrt{n}$ of Bob's indices are approximated to have mass less than $\frac{1}{2\sqrt{n}}$.
we will show that this implies that $\eps$ must be large.
In this case, the error incurred by the streaming algorithm will be
\[
    \left(\frac{1}{\sqrt{n}} - \frac{1}{2\sqrt{n}}\right) c\sqrt{n} = \frac{c}{2}.
\]
So, if $\eps < \frac{c}{2}$, then the reduction will correctly identify when $x_i = 0$ as many of Bob's indices must be predicted to have large mass. 
    
\paragraph{Case 2: $x_i = 1$.}
In this case, consider the two piece histogram that simply uses 1 piece and predicts mass $1/n$ everywhere. This gives an upper bound on $opt_2(S)$ (and for our setting of $a, b$ should actually be optimal).
\[
    opt_2(S) \leq \left(\frac{1}{\sqrt{n}} - \frac{1}{n}\right) b\sqrt{n} \leq b
\]

Assume that at least $c\sqrt{n}$ of Bob's indices are approximated to have mass at least $\frac{1}{2\sqrt{n}}$. We will show that this implies $\eps$ must be large.
Note that in this case, at least $(c - k)\sqrt{n}$ of Bob's indices must be covered by a histogram piece with height at least $\frac{1}{2\sqrt{n}}$ that also covers some other of Bob's indices (assuming $c > k$).
Thus, there must be $(c - k)\sqrt{n} \cdot \frac{a}{b}$ of Alice's elements which are predicted to have mass at least $\frac{1}{2\sqrt{n}}$.
So, the error of the streaming algorithm's approximation is at least
\[
    \left(\frac{1}{2\sqrt{n}} - \frac{1}{n}\right) \left(\frac{a}{b}\right)(c - k)\sqrt{n}
    = \frac{a(c - k)}{2b} - o(1).
\]
As we are guaranteed that the stream error is at most $opt_2(S) + \eps$, the reduction will correctly identify $x_i = 1$ as long as
\[
    \eps < \frac{a(c-k)}{2b} - b.
\]

It remains to give reasonable settings for the constants $a, b, c, k \in [0,1]$ under the following constraints
\begin{itemize}
    \item $a + b \leq 1$
    \item $a / b \in \mathbb{Z}$
    \item $b > c$
    \item $c > k$
    \item $\eps < \min\{\frac{c}{2}, \frac{a(c-k)}{2b} - b\}$
\end{itemize}

Set $a = \frac{1}{2}, b = \frac{1}{8}, c = \frac{1}{10}, k = \frac{1}{40}$.
Then, the bound on $\eps$ becomes
\[
    \eps < \min\{\frac{1}{20}, \frac{1}{40}\} = \frac{1}{40}.
\]

For this parameter regime, any streaming algorithm on domain size $n$ that outputs a histogram approximation with at most $\sqrt{n}/40$ pieces with error $opt_2(S) + \eps$ for $\eps < 40$ can be used to solve augmenting indexing on $\sqrt{n}$ bits and thus must use $\Omega(\sqrt{n})$ space.

\end{proof}


==> sampling.tex <==

\section{\texorpdfstring{$L_0$}{} and \texorpdfstring{$L_1$}{} sampling lower bound}

\paragraph{Setup}
We will consider algorithms that have the following query access to the target distribution $P$:
\begin{enumerate}
    \item \textbf{$L_1$ sampling with evaluation:} The algorithm can sample a point $i \sim P$ and will get the sample identity as well as the mass of $i$ under the distribution $P(i)$. (This can be implemented with errors in the streaming setting.)
    \item \textbf{$L_0$ sampling:} The algorithm can sample a point uniformly over $P$'s support $i \sim supp(P)$.
\end{enumerate}

\paragraph{Improper learning goal}
Return some function $f: [n] \rightarrow \mathbb{R_+}$ such that with probability at least $2/3$,
\begin{equation}
    \sum_{i \in supp(P)} |f(i) - P(i)| \leq \sum_{i \in supp(P)} |OPT_k(i) - P(i)| + \eps
\end{equation}
where $OPT_k(i)$ is the optimal $k$-piece piecewise constant function.

\paragraph{Lower bound}
Construction:
\begin{itemize}
    \item The first $n/2$ elements are ``mice'' (have mass $1/n$).
    \item Uniformly at random place $\sqrt{n}/2-1$ ``elephants'' (mass $1/\sqrt{n}$) among the last $n/2$ elements. Let $(e_1,e_2,\ldots,e_{\sqrt{n}/2-1})$ be the set of elephant locations ordered left to right.
    \item Uniformly at random pick an element $e$ in $(e_1,e_2,\ldots,e_{\sqrt{n}/2-2})$ and fill in all the remaining $\frac{1}{2\sqrt{n}}$ mass uniformly among the elements between $e$ and its successor (closest element to the right with nonzero mass). We will call these filled in elements ``hidden mice'' (note that these elements are only mice-sized with high probability).
    \item If $e$ and $e+1$ are elephants, instead fill in the remaining mass anywhere (we will argue that this happens with very small probability).
    % \item Uniformly at random place a contiguous block of $\sqrt{n}/2$ mice (mass $1/n$) among the last $n/2$ elements, ignoring the elephants (pretend that the elephant elements don't exist).
\end{itemize}
Note that this is a valid family of distributions over the domain $[n]$ (namely, the total mass is $1$).
Also note that this distribution can always be fit with zero error by a $4$-piece histogram $f$ defined as follows.
Let $i_{left}$ and $i_{right}$ be the boundary elephants around the hidden mice. The construction assumes that $i_{right} - i_{left} >1$, otherwise it is similar. \Piotr{To avoid dividing by zero}
\[
f(i) =
\begin{cases}
    1/n, &\text{for } i \in \{1,\ldots,n/2\} \\
    1/\sqrt{n}, &\text{for } i \in \{n/2+1,\ldots,i_{left}\} \\
    1/\left(2\sqrt{n}(i_{right}-i_{left} - 1)\right), &\text{for } i \in \{i_{left}+1,i_{right}-1\} \\
    1/\sqrt{n}, &\text{for } i \in \{i_{right},n\}
\end{cases}
\]

\begin{theorem}
Let $A$ be an improper density estimation algorithm that has $L_1$ and $L_0$ access to a distribution $P$ drawn from the family of distributions described above.
Then there exists some constant $C$ s.t. if $A$ draws at most $\sqrt{n}/C$ samples, $A$ cannot achieve estimation error less than $1/26$ with success probability $3/4$.
\end{theorem}

The proof has the following logical steps:
\begin{enumerate}
    \item Whp, there are $\sim \sqrt{n}$ hidden mice, each with mass $\sim 1/2n$. Conditioned on this, whp with $\sqrt{n}/C$ samples, neither $L_0$ nor $L_1$ sampling will find any hidden mice.
    \item $\sqrt{n}/C$ samples will only find a small fraction of the $\sqrt{n}/2$ elephants.
    \item The algorithm cannot at the same time incur low error with high probability on both the hidden mice and the unseen elephants.
\end{enumerate}

\begin{proof}
We will first argue that with high constant probability, the number of hidden mice is close to $\sqrt{n}$.
Recall that there are $\sim \sqrt{n}/2$ elephants uniformly placed in $n/2$ elements.
Let $e$ be the elephant we select as the left boundary for the hidden mice.
The probability that there is no elephant within the next $\sqrt{n}/10$ elements is (approximately)
\[
    \left(1 - \frac{\sqrt{n}/10}{n/2}\right)^{\sqrt{n}/2} \approx e^{-1/10} > 9/10.
\]
The probability that there are no elephants within the next $3\sqrt{n}$ elements is (approx)
\[
    1 - \left(1 - \frac{3\sqrt{n}}{n/2}\right)^{\sqrt{n}/2} \approx 1 - e^{-3} > 9/10.
\]
So, with probability at least $4/5$, the number of hidden mice is within $[\sqrt{n}/10, 3\sqrt{n}]$ with corresponding mass in $\left[\frac{5}{n}, \frac{1}{6n}\right]$.

%The number of hidden mice corresponds to number of balls in a randomly picked bin where we have $n/2 - (\sqrt{n}/2 - 1) \approx n/2 - \sqrt{n/2}$ balls and $\sqrt{n}/2-1 \approx \sqrt{n}/2$ bins.\Piotr{?}
%By symmetry we can just consider the number of balls in bin 1:
%\[
%    \E[\text{balls in bin 1}] = \frac{n/2 - (\sqrt{n}/2)}{\sqrt{n}/2} = \sqrt{n} - 1 \approx \sqrt{n}.
%\]
%By Chernoff bound,
%\[
 %   \Pr(\text{balls in bin 1} \notin \left[\frac{\sqrt{n}}{2}, \frac{3\sqrt{n}}{2}\right]) \leq 2e^{-\sqrt{n}/12}.
%\]
%\Piotr{I don't think this is true - the probability of having two elephants in a row is around $1/\sqrt{n}$}
%So, with high probability, the number of hidden mice is in the range $\left[\frac{\sqrt{n}}{2}, \frac{3\sqrt{n}}{2}\right]$ with corresponding mass in $\left[\frac{1}{n}, \frac{1}{3n}\right]$. 

Now, we will argue that we will sample none of the hidden mice with high probability conditioned on the number of hidden mice being in this range.
Note that there are at most $n/2 + \sqrt{n}/2 - 1 + 3\sqrt{n} < n/2 + 4\sqrt{n}$ supported elements.
Using $L_0$ sampling, the probability that we do not sample any of the last $n/2$ elements is at least
\[
    \left(1 - \frac{4\sqrt{n}}{n/2 + 4\sqrt{n}}\right)^{\sqrt{n}/C} \geq \left(1 - \frac{8}{\sqrt{n}}\right)^{\sqrt{n}/C} \geq 1 - \frac{8\sqrt{n}/C}{\sqrt{n}} = 1 - \frac{8}{C}
\]
(last inequality from \url{https://en.wikipedia.org/wiki/Bernoulli's_inequality}).
Using $L_1$ sampling, the probability that we do not sample any of the hidden mice (taking up $\frac{1}{2\sqrt{n}}$ mass) is
\[
    \left(1 - \frac{1}{2\sqrt{n}}\right)^{\sqrt{n}/C} \geq 1 - \frac{\sqrt{n}/C}{2\sqrt{n}} = 1 - \frac{1}{2C}.
\]
By union bound, the probability that we see any hidden mice with any combination of $L_0$ and $L_1$ sampling conditioned on reasonable numbers of hidden mice is at most $\frac{17}{2C}$.
Therefore, the marginal probability that we sample any hidden mice is at most 
\[
    \frac{17}{2C}\cdot \frac{9}{10} + 1 \cdot \frac{1}{10} = \frac{153}{20 C} + \frac{1}{10} < \frac{8}{C} + \frac{1}{10}.
\]
With constant probability, we will not see any of the hidden mice via sampling.
\Justin{check from under here}

As we take only $\sqrt{n}/C$ samples, we will see at most a $2/C$ fraction of the elephants, deterministically.
The algorithm $A$ will need to assign some values to the other $\geq n/2 - \sqrt{n}/C$ elements in the second half of the domain, guessing the positions of the unseen elephants and the hidden mice.

We will argue that the algorithm cannot both predict small values for the hidden mice and large values for the unseen elephants with good probability.
Specifically, let $i_{left}$ be the position of the left boundary elephant of the hidden mice.
We will say the algorithm gives \emph{$(\alpha,\beta)$ good mice predictions} if it predicts that at most $\alpha\eps\sqrt{n}$ of $\sqrt{n}/2$ elements directly to the right of $i_{left}$ have value greater than or equal to $\frac{1}{\beta\sqrt{n}}$.
Conditioned on the number of hidden mice being in $\left[\frac{\sqrt{n}}{2}, \frac{3\sqrt{n}}{2}\right]$, if the algorithm does not give good mice predictions, then the error will be at least
\[
    \alpha \eps\sqrt{n} \left(\frac{1}{\beta \sqrt{n}} - \frac{1}{n}\right)
    = \frac{\alpha \eps}{\beta} - \frac{\alpha \eps}{\sqrt{n}} > \frac{(\alpha-1)}{\beta}\eps.
\]

We will say the algorithm gives \emph{$(\gamma, \eta)$ good elephant predictions} if it predicts that at most $\gamma \eps\sqrt{n}$ of the unseen elephants have value less than or equal to $\frac{1}{\eta \sqrt{n}}$.
If the algorithm does not give good elephant predictions, then the error will be at least
\[
    \gamma \eps\sqrt{n}\left(\frac{1}{\sqrt{n}} - \frac{1}{\eta \sqrt{n}}\right)
    = \gamma \eps \left(1 - \frac{1}{\eta}\right)
\]

We will proceed by cases to show that the algorithm cannot give good predictions to the hidden mice and large predictions to the unseen elephants simultaneously.
\begin{enumerate}
    \item[\textbf{Case 1}] Algorithm $A$ gives $(\alpha, \beta)$ good mice predictions w.p.\ at least $2/3$. \\
    Conditioned on the seen elephants, the unseen elephants are distributed uniformly across the remaining second half of the domain.
    Note that the left boundary elephant is one of these unseen elephants with probability $(1 - 2/C)$.
    In order for $A$ to give good mice predictions, at least $2/3 (1 - 2/C)$ of these unseen elephants must have at least a $\left(1 - 2\alpha \eps\right)$ fraction of its following $\sqrt{n}/2$ elements being assigned small values ($\leq 1/\beta\sqrt{n}$).
    If $C > 20$, at least a $3/5$ fraction of the unseen elephants must have this property.
    
    Say that a $p$ fraction of the unseen second half of the domain is assigned small values.
    If $p$ is less than $3/5\left(1 - 2\alpha\eps\right)$, then the probability that the an unseen left boundary elephant has enough small values is less than $3/5$.
    Therefore, $p \geq 3/5\left(1 - 2\alpha\eps\right)$.
    
    \item[\textbf{Case 2}] Algorithm $A$ gives $(\gamma, \eta)$ good elephant predictions w.p.\ at least $2/3$. \\
    Recall that conditioned on the seen elephants, the unseen elephants are distributed uniformly across the remaining second half of the domain.
    If we assign small values ($\leq \frac{1}{\eta\sqrt{n}}$) to a $p$ fraction of the unseen second half of the domain, the expected number of unseen elephants assigned small values will be at least 
    \[
        p\left(\frac{\sqrt{n}}{2} - \frac{\sqrt{n}}{C} - 1\right) \geq p\sqrt{n}/3
    \]
    as long as $C > 7$.
    Let $X_i$ be an indicator r.v.\ for whether unseen elephant $i$ is assigned a small value.
    Note that the $X_i$'s are negatively correlated: if one unseen elephant gets assigned a small value, it means it took up one of the fixed number of small value slots.
    Therefore, we can apply a Chernoff bound:
    \[
        \Pr\left(\sum X_i < p\sqrt{n}/4\right) < e^{-p\sqrt{n}/96}.
    \]
    In order for $A$ to give $(\gamma, \eta)$ good elephant predictions with $3/4$ probability, $p$ must be less than $6\eps\gamma$.
    Otherwise, by the bound above, with high probability more than $\gamma\eps\sqrt{n}$ unseen elephants will have small values.
\end{enumerate}
From the two cases, we know the following bound on the fraction of small elements $p$:
\[
    \frac{3}{5}(1-2\alpha\eps) \leq p < 6\gamma\eps.
\]
Let's pick $\beta=\gamma=2$.
Then, $\alpha \leq 3$ and $\gamma \leq 2$ in order to achieve error at most $\eps$.
Therefore,
\[
    \frac{3}{5}(1-6\eps) < 12\eps
\]
and
\[
    \eps > \frac{1}{26}.
\]
Therefore, we cannot get estimation error better than $1/26$.

We end the proof by showing that we cannot achieve this estimation error with success probability $3/4$.
Recall that we have showed the following:
\begin{itemize}
    \item The probability that we do not sample any hidden mice is at most $\frac{3}{C}$.
    \item Conditioned on not seeing any hidden mice, we cannot get good mice and elephant predictions with probability at least $2/3$ (for some specific notion of good).
    \item If there are at least $\sqrt{n}/2$ hidden mice, this means that we cannot achieve estimation error $\eps=1/26$ with $2/3$ success probability.
    \item There are at least $\sqrt{n}/2$ hidden mice with probability $1 - O(1/\sqrt{n})$.
\end{itemize}
Let $C = 60$.
Then, even if $A$ gives perfect estimation if it sees any hidden mice or if the number of hidden mice is greater than $\sqrt{n}/2$, it still cannot give estimation better than $\eps=1/26$ with success probability $3/4$.
% Choosing $\eps = 1/50$ and $C = 20$, we get that in either case, if we achieve error $\leq \eps$ on either the hidden mice or the unseen elephants, we achieve error $> \eps$ on the other.
\end{proof}


==> sgd.tex <==

% \newpage
\section{SGD formulation}
\paragraph{Setup}
\begin{itemize}
    \item Given stream of $n$ elements from $[m]$ with true frequencies $f_i$ for $i \in [m]$.
    Let $S = \{i: f_i > 0\}$ be the support of the stream. 
    \item It will be useful to consider the normalized frequencies $p_i = \frac{f_i}{n}$.
    \item The loss of a linear model described by parameters $(a, b)$ is defined as
    \[
        L(a, b) = \frac{1}{|S|} \sum_{i \in S} [(ai + b) - p_i]^2.
    \]
\end{itemize}

\paragraph{Error}
\begin{itemize}
    \item From the lower bound, we know that it is impossible to approximate $L(a, b)$ up to any multiplicative factor using sublinear space.
    \item One notion of error that we might be able to say something about is the loss wrt the optimal linear loss:
    \[
        L^* - L(a, b)
    \]
    where $L^*$ is defined as
    \[
        L^* = \min_{a, b} L(a,b).
    \]
\end{itemize}

\paragraph{``SGD'' framework}
\begin{itemize}
    \item Initialize $a, b =0$ and set a learning rate $\eta$.
    \item Split the stream into $n/b$ batches of size $b$.
    \item For each batch $B$
    \begin{enumerate}
        \item Let $g_i$ be the number of times $i$ appears in $B$ and let $q_i = \frac{g_i}{b}$ be the ``normalized frequencies'' of the buffer.
        Also, let $S_B = \{i: g_i > 0\}$ be the support of $B$.
        \item We define the loss across $B$ to be
        \[
            L_B(a, b) = \frac{1}{|S_B|} \sum_{i \in S_B} [(ai + b) - q_i]^2.
        \]
        \Justin{There needs to be some added accounting for the fact that the $q_i$'s have much higher magnitude than the $p_i$'s due to the small support of $B$.}
        \item Run gradient updates for $a$ and $b$:
        \[
            a := a - \eta \left(\frac{1}{|S_B|} \sum_{i \in S_B} 2i[(ai + b) - q_i]\right)
        \]
        \[
            b: = b - \eta \left(\frac{1}{|S_B|} \sum_{i \in S_B} 2[(ai + b) - q_i]\right)
        \]
    \end{enumerate}
\end{itemize}

\paragraph{Random order}
Assuming random order, how are the batch frequencies $g_i$ distributed?
\[
    (g_1, g_2,...,g_m) \sim Multinomial(b, (p_1,p_2,...,p_m))
\]

\subsection{Poisson regression}
\paragraph{Setup}
\begin{itemize}
    \item Independent variable $X \in \mathbb{R}^d$
    \item Dependent variable $Y \in \mathbb{R}$
    \item Modeling assumption: $Y|X \sim Poi(f(X))$
    \item Extensive statistical analysis of the case where $f(X) = exp(\theta^T X)$, $\theta \in \mathbb{R}^d$
    \item To optimize, calculate the log likelihood $\log L(\theta | X, Y)$ and use gradient descent to find maximum likelihood $\theta$.
\end{itemize}

\paragraph{Interpretation in streaming model}
\begin{itemize}
    \item $X_i \in \mathbb{R}$ is the item key for element $i$
    \item $Y_i$ is the frequency of item $i$ over a fixed length of time
    \item Assume that $Y_i|X_i \sim Poi(f(X_i))$, each item shows up according to some fixed rate that is a function of $X_i$
    \item Equivalently (I think), we pick a random batch size distributed like $Poi(s)$ and say that $Y_i$ is the frequency of item $i$ in the batch.
    Then, $Y_i|X_i \sim Poi(f(X_i))$ if each element in the stream is picked i.i.d.\ from a discrete distribution over items.
    \item Then, our goal is to recover $f(X)$, the expected value of $Y_i | X_i$. This is exactly the problem above where each batch gives us a sample pair $X_i, Y_i$ for each item $i$ in our support.
\end{itemize}


\iffalse
\item \textbf{Case 1:} Algorithm $A$ gives $\alpha, \beta$ good mice predictions w.p.\ at least $2/3$. \\
    In order to achieve this, $A$ must assign ``small'' values $\leq 1/2\sqrt{n}$ to at least $1 - 3\eps \sqrt{n}$ of the mice.
    Otherwise, those $3\eps\sqrt{n}$ mice will contribute error at least
    \[
    3\eps\sqrt{n} \left(\frac{1}{2\sqrt{n}} - \frac{1}{n}\right) > \frac{3\eps\sqrt{n}}{3\sqrt{n}} = \eps.
    \]
    \Justin{fix from here}
    This corresponds to at least a $1 - \frac{3\eps\sqrt{n}}{\sqrt{n}/2} = 1-6\eps$ fraction of the hidden mice which must be assigned small values.
    
    \Justin{Can this be removed?}
    In order to argue about independence, it will be useful to ignore the possibility that the hidden mice occur in the interval preceding the $\leq \sqrt{n}/C$ seen elephants. 
    As the hidden mice precede a uniformly random elephant, this only occurs with probability $2/C$, so we can safely ignore this possibility.
    
    Then, we can view the hidden mice as being placed uniformly at random within the remaining elements, of which there are at least 
    \[
        XXX
    \]
    
    As the hidden mice as placed uniformly at random in a contiguous block, in order for $A$ to assign small values to a $1 - 6\eps$ fraction of the hidden mice with probability at least $2/3$, $A$ must assign small values to at least a $\frac{2}{3}(1 - 6\eps)$ fraction of the second half of the domain.
    
    Then, with high constant probability \Justin{fill in details}, at least $1/2$ of the unseen elephants will be assigned small values, contributing error
    \[
        \frac{1}{2}\left(\frac{\sqrt{n}}{2} - \frac{\sqrt{n}}{C}\right) \frac{1}{2\sqrt{n}} \geq \frac{\sqrt{n}/3}{4\sqrt{n}} = 1/12.
    \]
    
    \item \textbf{Case 2:} $A$ achieves error at most $\eps$ w.p.\ at least $2/3$ on the unseen elephants. \\
    In order to achieve this, $A$ must assign ``large'' values $\geq 1/2\sqrt{n}$ to at least $1 - 3\eps \sqrt{n}$ of the unseen elephants.
    This corresponds to a $1 - \frac{3\eps\sqrt{n}}{\sqrt{n}/2 - \sqrt{n}/{C}} \geq 1 - 9\eps$ fraction of the unseen elephants.
    In order to assign large values to this many elephants with probability at least $2/3$, $A$ must assign large values to at least a $1 - 18\eps$ fraction of the elements in the second half of the domain. \Justin{fill in details}
    
    By pigeonhole principle, at least $5/6$ of the contiguous intervals where hidden mice could be placed have at least a $1 - 3\eps$  of large values, contributing error $> \eps$ \Justin{check}.
    \fi
    
\newpage


==> twopasslower.tex <==
% \newpage
\section{Multi-pass lower bound}
\subsection{Hierarchy of candidate hard problems}
\paragraph{Communication model.} We use a multi-player cyclic communication framework: a single round of communication between $k$ players $P_1,\ldots,P_k$ starts with $P_1$ sending a message to $P_2$, proceeds with $P_2$ sending a message to $P_3$, and so on, until $P_k$ sends a message to $P_1$, concluding the communication round. In an $r$-round protocol, $P_1$ needs to announce the output at the end of round $r$.

\paragraph{Candidate hard problems.}
Next we define a hierarchy of multi-player augmented indexing problems (generalizing the usual augmented indexing problem), which we hypothesize to be hard in this communication setting as long as the number of rounds is strictly smaller than the number of players. 

\begin{definition}[multi-player folding]
Let $F=F(x_1,\ldots,x_k)$ be a $k$-player communication problem.
Its $n$-folded version, denoted $F^n=F^n(x_1,\ldots,x_{k+1})$, is a $(k+1)$-player communication problem defined as follows:
\begin{itemize}
  \item Each of the first $k$ players, $P_i$ for $i\in[k]$, gets $n$ inputs to $F$, denoted $x_i^1,...,x_i^n$.
  \item Player $P_{k+1}$ gets an input index $j\in[n]$, and as augmentations, $\{x_i^p\}$ for all $i=1\ldots k$ and $p<j$.
  \item Their goal is to compute $F(x_1^j ,\ldots, x_k^j)$.
\end{itemize}
\end{definition}
In words: The first $k$ players get $n$ instances of $F$, the last player gets the index of the instance they need to solve, and as augmentations, the inputs to all the preceding instances.

We now apply this definition inductively. Let $n>0$ be a fixed integer. As the induction base we use a ``vacuous'' single player communication problem, where the only plaeyr $P_1$ has a single input bit and needs to report it without any communication. Denote this problem by $F_1^{(n)}$ (even though this problem definition is independent of $n$). Now, for every $k>1$, let $F_k^{(n)}$ denote the $100^{k-1}n$-folded version of $F_{k-1}^{(n)}$. Note that $F_k^{(n)}$ is a $k$-player problem, in which the input of $P_1$ is of size $100^{(k-1)(k-2)/2}n^{k-1}=2^{\Theta(k^2)} n^{k-1}$ bits.

We observe that $F_2^{(n)}$ is simply the usual $n$-bit binary augmented indexing problem. For concreteness, let us also write out the problem $F_3^{(n)}$:
\begin{itemize}
  \item Alice has $100n$ bitstrings $a_1,\ldots,a_{100n}$ of length $n$ each (and we think of each as an instance of augmented indexing).
  \item Bob has $100n$ indices $b_1,\ldots,b_{100n}\in[n]$, and as augmentations, $a_i[1,\ldots,b_i-1]$ for every $i=1,\ldots,{100n}$.
  \item Charlie has an index $j\in[100n]$, and as augmentations,
  \begin{itemize}
    \item Augmentation from Alice: $a_i$ for every $i<j$.
    \item Augmentation from Bob: $b_i$ for every $i<j$ (and also $a_i[1,\ldots,b_i-1]$, but that's already contained in augmentations from Alice).
  \end{itemize}
  \item The required output is $a_j[b_j]$.
\end{itemize}

\paragraph{Conjectured hardness.}
In our multi-player cyclic communication model, we say that a randomized communication protocol  ``solves'' a problem if it returns the correct output with probability at least $2/3$, and that it ``uses $b$ bits'' if the largest message sent by any player in any round is of size $b$ bits.

\begin{conjecture}
For every $2\leq k=O(1)$, any $(k-1)$-round protocol that solves $F_k^{(n)}$ must use $\Omega(n)$ bits. 
\end{conjecture}

A possible way to prove it is by the following elimination lemma (whose proof is incomplete).
\begin{lemma}[conjectured round/player elimination lemma]
Let $k\geq2$. If there is a $k$-round protocol that solves $F_{k+1}^{(n)}$ using $b$ bits, then there is a $(k-1)$-round protocol that solves $F_k^{(n)}$ using $O(b)$ bits. 
\end{lemma}
The lemma immediately implies the conjecture, due to the known $\Omega(n)$ lower bound for single round $n$-bit augmented indexing, which is $F_2^{(n)}$.

We attempt to prove the lemma by adapting the proof of the original (two player) round elimination lemma. The following is a proof of the lemma given a claim formulated below as \cref{clm:missing}. What remains is to prove the claim (if true).

\begin{proof}
Since we recall that $F_{k+1}^{(n)}$ is the $100^kn$-folded version of $F_k^{(n)}$, it will be convenient to denote $N=100^kn$.

By Yao, it suffices to show that for every distribution $D$ on inputs $\{\mathbf x=(x_1,\ldots,x_k)\}$ to $F_k^{(n)}$, there is a deterministic $(k-1)$-round protocol that uses $O(b)$ bits (where the hidden constant does not depend on $D$) and is correct for $F_k^{(n)}$ with probability at least $2/3$ over $D$. 

Let $D^N$ the $N$-times product distribution of $D$ (i.e., drawing a sequence of $N$ independent samples of $D$). We define a distribution $D^*$ over inputs to $F_{k+1}^{(n)}$ as the product distribution $D^N\times\textrm{Uniform}[N]$. That is, $D^*$ is defined by drawing $N$ independent samples $\{\mathbf x^p=(x_1^p,...,x_k^p):p\in[N]\}$ from $D$, and independently of them sampling $j\in[N]$ uniformly at random. Note that as per the definition of folding above, this is indeed an input to $F_{k+1}^{(n)}$ (where each player $i=1,\ldots,k$ gets $\{x_i^p:p\in[N]\}$ as input, and player $k+1$ gets $j$ as input).

The premise of the lemma is that we have a $k$-round protocol that solves $F_{k+1}^{(n)}$ using $b$ bits. Assume w.l.o.g.~that its failure probability is $1/200$ (we can amplify its success probability by taking the majority of a constant number of parallel executations, and this only changes $b$ by a constant, which we can suppress into the $O(\cdot)$ notation in the lemma statement). By Yao, this means there is a deterministic protocol, denoted henceforth by $\Pi^*$, that uses $b$ bits and returns the correct output for $F_{k+1}^{(n)}$ with probability at least $199/200$ over $D^*$.

Let $R$ be the subset of the support of $D^N$ that contains the elements $(\mathbf x^1,\ldots,\mathbf x^N)$ such that $\Pi^*$ returns the correct output on input $((\mathbf x^1,\ldots,\mathbf x^N),j)$ for at least a 0.99 fraction of the $j$'s in $[N]$, or in other words,
\[ R = \{(\mathbf x^1,\ldots,\mathbf x^N)\in\mathrm{support}(D^N) : \Pr_{j\sim[N]}\left[\Pi^*((\mathbf x^1,\ldots,\mathbf x^N),j) \text{ is correct for } F_{k+1}^{(n)}\right] \geq 0.99 \} . \]

We observe that the fact that $\Pi^*$ succeeds on inputs from $D^*$ with probability at least $199/200$ implies that $\Pr_{y\sim D^N}[y\in R]\geq1/2$. This is because we can write
\begin{align*}
  &\Pr_{(y,i)\sim D^*}[\Pi^*(y,i)\text{ succeeds}] \\
  &= \Pr_{(y,i)\sim D^*}[\Pi^*(y,i)\text{ succeeds}|y\in R]\Pr_{y\sim D^N}[y\in R] + \Pr_{(y,i)\sim D^*}[\Pi^*(y,i)\text{ succeeds}|y\notin R]\Pr_{y\sim D^N}[y\notin R] \\
  &< \Pr_{y\sim D^N}[y\in R] + 0.99\cdot(1-\Pr_{y\sim D^N}[y\in R]),
\end{align*}
and this is less than $0.995=199/200$ if $\Pr_{y\sim D^n}[y\in R]<1/2$.

At the end of the first round of $\Pi^*$, the last player $P_{k+1}$ sends the first player $P_1$ a message of size at most $b$ bits, thus partitioning $R$ into at most $2^b$ subsets. Of them, let $T$ be the subset with maximal mass w.r.t.~$D^n$, i.e., the one that maximizes $\Pr_{(\mathbf x^1,\ldots,\mathbf x^N)\sim D^N}[(\mathbf x^1,\ldots,\mathbf x^N)\in T]$. Then we have
\[ \Pr_{y\sim D^N}[y\in T] \geq \frac{1}{2^b}\cdot\Pr_{y\sim D^N}[y\in R] \geq \frac1{2^{b+1}} . \]

To proceed, let us introduce the notation $\mathcal I_i$ for the set of possible inputs to player $i$ in the problem $F_k^{(n)}$. We can now formulate our missing claim.
\begin{claim}\label{clm:missing}
The following exist:
\begin{itemize}
  \item $j\in[N]$,
  \item $j-1$ inputs $\{\mathbf z^p=(z_1^p,\ldots,z_k^p):p=1,\ldots,j-1\}$ to $F_k^{(n)}$,
  \item a subset $G$ of inputs to $F_k^{(n)}$ with $D$-mass at least $0.9$, i.e., such that $\Pr_{\mathbf x\sim D}[\mathbf x\in G]\geq0.9$,
  \item maps $f_i^p:\mathcal I_i\rightarrow\mathcal I_i$ for every $i\in[k]$ and $p\in\{j+1,\ldots,N\}$, 
\end{itemize}
with the following property: For every input $\mathbf x=(x_1,\ldots,x_k)$ to $F_k^{(n)}$ which is contained in $G$, if for every $p=j+1,\ldots,N$ we denote $\mathbf f^p=(f_1^p(x_1),\ldots,f_k^p(x_k))$ (this is an input to $F_k^{(n)}$), then we have both of the following:
\begin{itemize}
  \item $(\mathbf z^1,\ldots,\mathbf z^{j-1},\mathbf x,\mathbf f^{j+1},\ldots,\mathbf f^N)\in T$, and
  \item $\Pi^*$ is correct for $F_{k+1}^{(n)}$ on the input $(\mathbf z^1,\ldots,\mathbf z^{j-1},\mathbf x,\mathbf f^{j+1},\ldots,\mathbf f^N,j)$.
\end{itemize}
\end{claim}

We now show that the claim implies the lemma. We describe a deterministic $(k-1)$-round protocol $\Pi$ for $F_k^{(n)}$. 
Given the input $\mathbf x=(x_1,\ldots,x_k)$ to $F_k^{(n)}$, each of the $k$ players $P_i$ for $i=1,\ldots,k$ pretends to have the input $(z_i^1,\ldots,z_i^{j-1},x_i,f_i^{j+1}(x_i),\ldots,f_i^N(x_i))$ to $F_{k+1}^{(n)}$. Player $P_k$ also takes it upon herself to simulate player $P_{k+1}$ with input $j$. This sets up an instance of $F_{k+1}^{(n)}$. The players now simulate $\Pi^*$ on those pretended inputs, skipping the first round, instead pretending that at the end of it, $P_{k+1}$ sent $P_1$ the $b$-bit message that defines $T$. Thus, it is a $(k-1)$-round protocol that uses $b$ bits.

Next we argue that $\Pi$ succeeds for $F_k^{(n)}$ with probability at least $0.9$ on a random input $\mathbf x$ drawn from $D$. This holds simply because $\mathbf x$ is contained in $G$ with probability at least $0.9$ by the claim, and furthermore by the claim, the pretended input of $F_{k+1}^{(n)}$ for the simulated $\Pi^*$ is contained in $T$. This means that the players were correct to assume the first round concluded with $P_{k+1}$ sending $P_1$ the message that defines $T$, so the remainder of the simulation of $\Pi^*$ remains faithful, and again by the claim we know that $\Pi^*$ is correct on the pretended input. This proves the lemma given the claim, and it only remains to prove the claim.
\end{proof}

\subsection{Reduction for 2-pass lower bound}

We now show that if the above conjectured hardness holds for $k=3$, then we have an $\Omega(n^{1/3})$ space lower bound for solving the 2-piece histogram problem up to error $\epsilon\cdot n^{2/3}$. Ideally, we want to amplify this to $\epsilon n$.

\begin{theorem}
If the above conjectured hardness is correct for $k=3$, then every $2$-pass algorithm that solves our histogram problem with $2$ pieces (proper learning) and with error up to $\epsilon\cdot n^{1/3}$ (where the total mass of the stream is $n$), must use $\Omega(n^{1/3})$ space.
\end{theorem}
\begin{proof}
We let $m=\Theta(n^{1/3})$, and we reduce from $F_3^{(m)}$ that was defined above. Alice, Bob and Charlie are given inputs to $F_3^{(m)}$.

\begin{itemize}

\item Alice's inputs are $100m$ bitstrings $a_1,\ldots,a_{100m}$ of length $m$. She partitions the size-$n$ domain of the stream into $100m$ parts $d_1,\ldots,d_{100m}$, one per $a_i$. Each $d_i$ has size $n/(100m)=\Theta(n^{2/3})=\Theta(m^2)$, so she can encode in it the 1-pass lower bound gadget for $a_i$ by streaming the appropriate mice. 

\item Bob's inputs are $b_1,\ldots,b_{100m}\in[m]$ plus the augmentations from Alice. In each $d_i$ he now encodes his own  response to the 1-pass lower bound gadget, with elephants of size $\Theta(m)$.

\item Charlie's input is $j\in[100m]$, and the augmentations from Alice and Bob. Using these augmentations, he can zero out (with deletions) everything in the domain parts $d_1,\ldots,d_{j-1}$. Furthermore, he encodes $C$ mice after domain part $d_j$, and $Cn$ mice at the end of the entire domain, where $C$ is a large constant.

\item Their goal is to report $a_j[b_j]$.
\end{itemize}

Now we argue that every algorithm that solves the $2$-piece histogram problem up to error $\epsilon\cdot n^{2/3}$ also solves this instance of $F_3^{(m)}$, yielding a lower bound of $\Omega(m)=\Omega(n^{1/3})$ as desired, under the conjectured hardness from the previous section. 

Recall (or observe) that the 1-pass lower bound gadget is constructed such that the optimal solution with a single piece histogram is to use one mouse piece. We then get zero error on the mice and $c'n$ error (for some constant $c'$) on the elephants. Thus here, the optimal solution with a single piece on each domain part $d_i$ is a mouse piece which yields error $cm^2$ (for some constant $c$). 

Consider the following 2-piece solution for the instance Alice, Bob and Charlie just constructed. We compute the optimal $2$-piece solution for part $d_j$, recalling (from the 1-pass lower bound proof) that this solution is an elephant piece followed by a mouse piece, and then stretch the mouse piece until the end of the domain. Then we get $cm^2$ error on each piece $d_{j+1},\ldots,d_{100m}$ and zero error on Charlie's mice, for a total error of $opt(d_j)+cm^2(100m-(j+1))$. Observe that since $m=\Theta(n^{1/3})$, this is at most $O(n)$. 

We claim this is the optimal 2-piece solution. The reason is that to get less than $cm^2$ error on any other part of domain (i.e., in parts $d_{j+1},\ldots,d_{100m}$), we need to use at least 2 pieces. This means that one of the two Charlie mice locations (right after $d_j$, and at the end of the domain) will generate at least $1$ unit of error per mouse, meaning at least $Cn$ error, more than the $O(n)$ above.

So, the optimal solution has value $opt(d_j)+cm^2(100m-(j+1))$. We recall from the 1-pass lower bound gadget that $opt(d_j)$ equals $0$ if $a_j[b_j]=0$, and equals $\Theta(\epsilon m^2)=\Theta(\epsilon\cdot n^{2/3})$ if $a_j[b_j]=1$. Thus, if we have an algorithm for the histogram problem which is accurate up to $\Theta(\epsilon\cdot n^{2/3})$, we have solved $F_3^{(m)}$.
\end{proof}
